Autoregressive Multi-trait Essay Scoring via Reinforcement Learning with Scoring-aware Multiple Rewards

Recent advances in automated essay scoring (AES) have shifted towards evaluating multiple traits to provide enriched feedback. Like typical AES systems, multi-trait AES employs the quadratic weighted kappa (QWK) to measure agreement with human raters, aligning closely with the rating schema; however, its non-differentiable nature prevents its direct use in neural network training. In this paper, we propose Scoring-aware Multi-reward Reinforcement Learning (SaMRL), which integrates actual evaluation schemes into the training process by designing QWK-based rewards with a mean-squared error penalty for multi-trait AES. Existing reinforcement learning (RL) applications in AES are limited to classification models despite associated performance degradation, as RL requires probability distributions; instead, we adopt an autoregressive score generation framework to leverage token generation probabilities for robust multi-trait score predictions. Empirical analyses demonstrate that SaMRL facilitates model training, notably enhancing scoring of previously inferior prompts.

==> fig/table_data.tex <==


\begin{table}[t]
\centering
\scalebox{
0.7}{
\begin{tabular}{c|c|l}
\hline
Prompt & \# Essays & Traits\\
\hline
1 & 1785 & Over, Content, WC, Org, SF, Conv \\
2 & 1800 & Over, Content, WC, Org, SF, Conv \\
3 & 1726 & Over, Content, PA, Nar, Lang \\
4 & 1772 & Over, Content, PA, Nar, Lang \\
5 & 1805 & Over, Content, PA, Nar, Lang \\
6 & 1800 & Over, Content, PA, Nar, Lang \\
7 & 1569 & Over, Content, Org, Conv, Style \\
8 & 723 & Over, Content, WC, Org, SF, Conv, Voice \\
\hline
\end{tabular}}
\caption{\label{tab1}
Composition of the ASAP/ASAP++ combined dataset. The prompt is an instruction that defines the writing theme. Over: \textit{Overall}, WC: \textit{Word Choice}, Org: \textit{Organization}, SF: \textit{Sentence Fluency}, Conv: \textit{Conventions}, PA: \textit{Prompt Adherence}, Nar: \textit{Narrativity}, Lang: \textit{Language}.}
\end{table}

==> fig/table_prompt.tex <==

\begin{table}[h]
\scalebox{
0.5}{
\centering
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}
\hline
Prompts & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & Avg \\ 
\hline
reg & 0.711 & 0.582 & 0.627 & 0.758 & 0.768 & 0.776 & 0.766 & 0.604 & 0.699 \\ 
\hline
cls & 0.666 & 0.579 & 0.653 & 0.758 & 0.781 & 0.786 & 0.711 & 0.491 & 0.678 \\ 
\hline
cls$_{penalty}$ & 0.666 & 0.579 & 0.662 & 0.761 & 0.786 & 0.787 & 0.726 & 0.525 & 0.687 \\ 
\hline
cls$_{penalty}$+RL & 0.680 & 0.589 & 0.670 & 0.771 & 0.796 & 0.798 & 0.737 & 0.545 & 0.698 \\ 
\hline
cls$_{di}$ & 0.759 & 0.630 & 0.673 & 0.768 & 0.795 & 0.790 & 0.748 & 0.536 & 0.712 \\ 
\hline
cls$_{di}$+RL & \textbf{0.766} & \textbf{0.659} & \textbf{0.688} & 0.778 & \textbf{0.805} & 0.791 & 0.760 & 0.545 & 0.724 \\ 
\hline
SaMRL (Ours) & 0.762 & 0.640 & 0.685 & \textbf{0.799} & 0.804 & \textbf{0.821} & \textbf{0.806} & \textbf{0.680} & \textbf{0.750} \\ 
\hline
\end{tabular}}
\caption{Comparison of Different Methods}
\end{table}

